Fault-tolerant Fusion-based Quantum Computing with the Four-legged Cat Code

The four-legged cat code is a quantum error-correcting code designed to address the predominant error in bosonic modes: single-photon loss. It was the first such code to surpass the break-even point, thereby demonstrating the practical utility of quantum error correction. In this work, we propose a planar fault-tolerant architecture for this code by concatenating it with the XZZX code via fusion-based error-correction. To the best of our knowledge, this is the first 2D nearest-neighbor architecture for fault-tolerant fusion-based error-correction. We demonstrate how all the required operations, namely resource state preparation and Bell measurements, can be carried out using standard circuit-QED techniques, such as intercavity beam-splitter coupling, cavity displacements, cavity-transmon dispersive coupling, and transmon drives. We show analytically and numerically that all dominant hardware errors in the bosonic modes and control ancillae are corrected, to first-order, at the hardware level. Consequently, the outer XZZX code only needs to address smaller residual errors, which are quadratically suppressed, effectively doubling the architecture's fault-distance. Moreover, the performance of our architecture is not limited by unwanted nonlinearities such as cavity self-Kerr, and it avoids demanding coupling techniques like $\chi$-matching or high-order coupling. Overall, our architecture substantially reduces the hardware complexity needed to achieve fault tolerance with the four-legged cat code.

==> tex/scratch.tex <==


%Our protocol relies on two fault-tolerant operations: heralded preparation of 6-body entangled resource states and destructive Bell measurements (fusions). We propose a planar architecture tailored for implementation with superconducting circuits and 3D microwave cavities. These operations are implemented using standard superconducting circuit techniques, such as intercavity beam-splitter coupling, cavity displacements, cavity-transmon dispersive coupling, and transmon drives.
% \hkb{Comment by Harsh}
% \jdt{James}
% \jc{Jahan}
% \rjs{Rob}
% \sp{Shruti}

%\tableofcontents

%%% Intro

%Traditional methods achieve leverage multiple noisy qubits to realize this redundancy \cite{shor_1995, steane_1996,kitaev_1997b, bravyi_1998, kitaev_2003, fowler_2012a}. An alternative approach embeds redundancy directly within a single physical mode, such as a harmonic oscillator \cite{cochrane_1999, gkp_2001, glancy_2004, braunstein_2005, weedbrook_2012, leghtas_2013, mirrahimi_2014, michael_2016, albert_2016, albert_2018, niu_2018, grimsmo_2020, albert_2022, schlegel_2022, hillmann_2023, korolev_2023}. 
%Entirely simulating these operations is computationally infeasible, thus we separately simulate portions of the circuit and bound the overall infidelity. We observe that hardware errors during fusions primarily affect the $ZZ$ measurement results. On the other hand, the $XX$ measurements are fundamentally limited by the size of the 4C states. This noise bias further motivates our choice of the $XZZX$ code, which offers a higher threshold compared to the standard surface code under such biased noise conditions \cite{wen_2003, kovalev_2011, ataides_2021, claes_2023, sahay_2023a}.

%%% Planar FBEC

%\hkb{Integrating these error-detected gates into a FBQC framework has two key benefits. First, despite the need to reinitialize the bosonic modes and retry the gate, we can implement a universal set of operations. This relaxes the hardware requirements by avoiding the need for error-corrected gates which demand intricate control techniques to ensure $\chi_{e,1} \approx \chi_{f,1}$ \cite{reinhold_theis_2019, rosenblum_2018, reinhold_2020, qian_xu_2023}. Second, the gate fidelity $\veps_{\text{pass}}$, is quadratically improved, scaling as $p_{\text{phys}}^2$, since two hardware errors are needed to bypass error detection during the gate \cite{tsunoda_2023}. }

%In Appendix \ref{app:planar_fbec_4star}, we present an alternative approach for FBEC based on the "4-star" resource states \cite{bartolucci_2023,sahay_2023a}. This approach involves simpler state-preparation circuits at the cost of more qubits. 


%%% Discussion 

%But we leave the exact estimation of the hardware overhead with this architecture and benchmark with other superconducting qubit architectures for future work.

%While single-mode bosonic codes have demonstrated impressive improvements in quantum memory lifetime, implementing error-corrected operations and achieving full fault-tolerance on these bosonic qubits has remained an enduring challenge. This work introduces a novel framework for achieving FT quantum computing using the four-legged cat code. The cat code is encoded within the electromagnetic mode of superconducting microwave cavities. These cavities are coupled to each other via tunable beamsplitters forming a planar lattice. Each cavity is dispersively coupled to a three-level ancilla, such as a transmon. Importantly, our protocol relies on well-established cQED tools, avoiding intricate techniques like $\chi$-matching, engineered dissipation, or multi-photon drives.

%Previous implementations of bosonic QEC have struggled with three critical issues: implementing FT entangling operations, correcting errors inherited from the coupled ancillae, and mitigating the state distortion from the no-jump evolution and parasitic non-linearities such as self-Kerr. Our work systematically tackles these challenges with a FT protocol to concatenate the cat code with the XZZX surface code using FBEC, relying on only three operations: error-detected GHZ state preparation, error-detected CZ gates, and FT fusion measurements. These operations are engineered to maintain the cat code's inherent robustness against single-photon loss (the dominant error mechanism in cavities) as well as to correct for a single ancilla decay or dephasing error. Furthermore, these operations suppress the effect of parasitic non-linearities, to first-order. Overall, any single dominant hardware error, whether in the bosonic mode or coupled ancillae, is prevented from propagating to the outer XZZX code, effectively doubling the distance of the outer code. 

%We propose a novel planar implementation of FBEC, which efficiently reuses previously measured qubits. FBEC is particularly well suited for the cat code as it counteracts damping effects from the no-jump evolution by frequently teleporting the logical information, eliminating the need for complex nonlinear interactions to stabilize the cat-code manifold. Additionally, we believe that these frequent measurements may also suppress coherent errors in the cat code \cite{sahay_2023b}. 

%Using current cQED hardware coherences, we project error-detected CZ gate infidelities %check again based on final simulations 
%below 0.01\% with a 1\% gate failure probability. Fusion measurements are expected to have a 1\% chance of incorrect $\op{Z}_\rmL \otimes \op{Z}_\rmL$ outcomes and a 0.1\% chance of incorrect $\op{X}_\rmL \otimes \op{X}_\rmL$ outcomes. This stands in contrast to the widely studied photonic cluster state \cite{browne_2005,devitt_2009,li_2010,bartolucci_2023,sahay_2023a}, where failure rates below 25\% demand increasingly challenging hardware \cite{li_2010,grice_2011}. Numerical simulations confirm that errors in each of our proposed operations scale quadratically with hardware coherences. Resource state preparation errors are orders of magnitude smaller than those during fusions, suggesting a phenomenological error model with approximately a 5\% threshold for the outer XZZX code \cite{claes_2023}. Our work suggests that this protocol may be a highly attractive candidate for FT quantum computing well below threshold using existing technology. However, more rigorous verification of the threshold for our particular error model remains to be explored in future work.

%Interestingly, hardware errors primarily affect $\op{Z}_\rmL \otimes \op{Z}_\rmL$ fusions more than $\op{X}_\rmL \otimes \op{X}_\rmL$ fusions. This bias could be exploited by the XZZX code as hardware coherences improve, further enhancing its threshold. Additionally, fusion errors could be reduced by converting all first-order errors into erasures. Erasures are especially favorable for the outer code, offering significantly higher thresholds and more favorable scaling with code distance \cite{wu_2022,sahay_2023a,chang_2024}. The quantitative study of these improvements is left for future work.  

%By seamlessly combining the four-legged cat code's robustness with the XZZX surface code's QEC capabilities, this work establishes a practical and experimentally feasible pathway toward scalable, FT quantum computers. The reliance on standard cQED techniques and hardware-level error detection makes this protocol not only accessible with current technologies but also a compelling candidate for FT quantum computing below threshold. We hope this work inspires new strategies for co-designing hardware-level operations and quantum error correction.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Scratch 
%  in two key directions. First, we enhance its robustness against errors that limited earlier experiments, including no-photon-jump backaction, errors inherited from ancillae, and unwanted non-linearities in the bosonic mode. Second, we propose a hardware-efficient architecture for arbitrary error suppression by concatenating the four-legged cat code with an outer XZZX code, leveraging fusion-based quantum computing (FBQC). Crucially, this protocol can be implemented using 
% 
% ------------
% 2: How you're doing everything
% a) 4cat challenges (which have limited prv) + solution with FBQC. 
% b) Hardware implementations: i.e. cqed tools. 
% In addition to FT, we address issues which limited the prev. experiment (as a tertiary point)
% 
% 3: Details as in what steps are + qualitative claims. Assumption: no dephasing. 
% 
% 4. quantitative \& include numbers.   
% 
% 5: Structure of the paper
% (up to 2nd page 1st col. only)
% 




%\hkb{major reworking - see SNAP paper or Ofek or Vlad Sivak's GKP papers for comparison with qubit-based codes. Then say that bosonic QEC is approximate, not fully FT. But can when concatenated with a larger QEC code, can achieve FT and hardware efficient. }

% from Kaavya's CNOT paper: In fixed-qubit architectures, the prominence of the surface code can be attributed to its 2D planar layout, nearest-neighbour connectivity, low-depth stabilization circuits, and high error tolerance threshold [20–22]. Efficient graph-based decoders, such as minimum weight-perfect matching (MWPM), perform well at correcting common circuit-level errors [23, 24]. Beyond these considerations, logical gates on surface codes are well understood and easy to implement with 2D nearestneighbor connectivity via braiding [20, 25, 26] or lattice surgery [27, 28].

% However, in practice, errors in gates are far from negligible and are likely to remain so for the forseeable future, so neglecting errors during the encoding and decoding circuits is a poor approximation.
% If we want to put together millions or more gates to perform a large quantum computation, the prospect of getting through the whole circuit without errors is vanishingly unlikely.
 
% To protect quantum computations against errors, we need something more than a quantum error correcting code, we need a fault-tolerant protocol, which allows us to perform unitary gates on encoded states despite errors occurring during the computation.
 
% In going from storage to computation one must begin to think of how errors propagate through the computing circuits. While an error correcting code might be designed to deal with a certain class of errors (e.g. single qubit errors), the action of doing computation can transform the errors to a new, larger, potentially uncorrectable set.

% Threshold theorem, which says that arbitrarily long quantum computations are possible provided the error rate per physical gate and time step is below some constant threshold value.
% If the physical operations are below a critical noise threshold, the logical error should be suppressed  exponentially as we increase the number of physical qubits per logical qubit. This behavior is expressed in the approximate relation

% Here, d is the code distance indicating 2d2 - 1 physical qubits used per logical qubit, p and epsd are the physical and logical error rates respectively, and pthr is the threshold error rate of the code. Thus, when p << pthr, the error rate of the logical qubit is suppressed



%Superconducting microwave resonators can be robustly constructed to have lifetimes that are an order of magnitude longer than the best Josephson junction-based qubits \cite{reagor_2013,reagor_2016, rosenblum_2018, reinhold_2020}. Furthermore, it is simpler to access the infinite-dimensional Hilbert space of these oscillators, making them an attractive candidate for hardware-efficient quantum error correction (QEC) \TODO{cite 4cats, binomial, GKP, others?}. The four-legged cat code is one such QEC code, that encodes a single logical qubit within a mode of a harmonic oscillator. 


% qian xu thesis Due to the highly nonlinear nature of the cat codes, implementing fault-tolerant logical operations is challenging. Existing schemes either require strong nonlinear interactions between bosonic modes (see e.g. [4, 59]), or use discrete-variable ancillae that could inject errors to the bosonic modes [75].
% Q.X thesis: One of the primary complexities stems from the weak non-linear interactions inherent in bosonic modes, necessitating the use of discrete-variable ancillae in systems such as circuit quantum electrodynamics (circuit QED) platform [123, 124]. However, a significant challenge arises in this hybrid system, as errors in the ancillae tend to propagate back to the bosonic mode, potentially compromising the encoded quantum information [125].
%But still major issue is ancilla FT - see Qian Xu's thesis, dual rail, Taka gates. So this is what we do. 
% \hkb{this can go at the end, tying together both concepts, i.e. using E.Dtctd to construct E.C.} Q.Xu: Consequently, while universal error-detection operations on bosonic qubits have been constructed [127, 128] and demonstrated [129], achieving a complete set of error-corrected operations has remained a significant challenge.
